Fast Arithmetic in Algorithmic Self-Assembly

In this paper we consider the time complexity of computing the sum and product of two $n$-bit numbers within the tile self-assembly model. The (abstract) tile assembly model is a mathematical model of self-assembly in which system components are square tiles with different glue types assigned to tile edges. Assembly is driven by the attachment of singleton tiles to a growing seed assembly when the net force of glue attraction for a tile exceeds some fixed threshold. Within this frame work, we examine the time complexity of computing the sum or product of 2 n-bit numbers, where the input numbers are encoded in an initial seed assembly, and the output is encoded in the final, terminal assembly of the system. We show that the problems of addition and multiplication have worst case lower bounds of $\Omega(\sqrt{n})$ in 2D assembly, and $\Omega(\sqrt[3]{n})$ in 3D assembly. In the case of addition, we design algorithms for both 2D and 3D that meet this bound with worst case run times of $O(\sqrt{n})$ and $O(\sqrt[3]{n})$ respectively, which beats the previous best known upper bound of O(n). Further, we consider average case complexity of addition over uniformly distributed n-bit strings and show how to achieve $O(\log n)$ average case time with a simultaneous $O(\sqrt{n})$ worst case run time in 2D. For multiplication, we present an $O(n^{5/6})$ time multiplication algorithm which works in 3D, which beats the previous best known upper bound of O(n). As additional evidence for the speed of our algorithms, we implement our addition algorithms, along with the simpler O(n) time addition algorithm, into a probabilistic run-time simulator and compare the timing results.

==> runTimeComparison.tex <==

\section{Parallel Time Versus Probabilistic Time}
In the case of large seed assemblies, simple examples show that probabilistic time can be a log factor faster than probabilistic time in the size of the seed.  To show that in general it is no worse, we provide the following bound.

\begin{lemma}
Consider a deterministic aTAM $\Gamma = (S,T,\tau)$ system that uniquely assembles $A$ in parallel run-time $t$.  Then $\Gamma$ assembles $A$ in probabilistic run-time $O(t\log(t + |S|))$.
\end{lemma}


\begin{lemma}
Let $X = \sum_{i=1}^{n} X_i$ be a random variable denoting the sum of $n$ independent exponentially distributed random variables with rate $\lambda$. Let $\mu = n/\lambda$ denote $E[X]$. Then $Pr[ X > (1+\delta)\mu ] < (\frac{\delta+1}{e^\delta})^n$.
\end{lemma}

\begin{proof}
 To achieve the upper bound on $X$ we apply the Chernoff bound technique described in \cite{XXX} to the case of exponentially distributed random variables.

 For any positive real $t$ we have that:

 $$Pr[X > (1+\delta)\mu] = Pr[exp(tX) > exp(t(1+\delta)\mu)].$$

 By applying the Markov inequality we get that:

 $$Pr[X > (1+\delta)\mu] < \frac{E[exp(tX)]}{exp(t(1+\delta)\mu)}.$$

 Note that $E[exp(tX)] = E[exp(t\sum_{i=1}^{n} X_i)] = E[\prod_{i=1}^{n} exp(tX_i)]$.  Further, as the $X_i$ are independant, we have that $E[\prod_{i=1}^{n} exp(tX_i)] = \prod_{i=1}^{n} E[exp(tX_i)]$.  We therefore get:

 $$Pr[X > (1+\delta)\mu] < \frac{\prod_{i=1}^{n} E[exp(tX_i)]}{exp(t(1+\delta)\mu)}.$$

 We now compute the value $E[exp(tX_i)]$.  For all $t$ such that $0 < t < 1$,

 $$ E[exp(tX_i)] = \int_0^{\infty} e^{tx}\lambda e^{-\lambda x} dx =  \lambda\int_0^{\infty} e^{x(t-\lambda)} dx = \frac{\lambda}{\lambda-t}.$$

 By plugging in this value for $E[exp(tX_i)]$ and replacing $\mu$ by $n/\lambda$, we get,

 $$Pr[X > (1+\delta)\mu] < (\frac{\lambda}{(\lambda-t) exp(\frac{t(1+\delta)}{\lambda}) })^n.$$

 Finally, we choose the $t$ that obtains the tightest bound by setting the derivative of the right hand side with respect to $t$ equal to 0. Solving this equation for $t$ gives $t= \frac{\lambda\delta}{\delta +1}$.  Plugging this value in for $t$ yields:

 $$Pr[X > (1+\delta)\mu] < (\frac{\delta+1}{e^\delta})^n.$$

\end{proof}


The following Lemma is essentially Lemma 5.2 from \cite{woods2012EAS}, slightly modified to be a statement about sums of exponentially distributed random variables, rather than a statement specific to the assembly model considered in the respective paper.

\begin{lemma}
Let $t_1 ,\ldots , t_m$ denote $m$ random variables where each $t_i = \sum_{j=1}^{k_i}t_{i,j}$ for some positive integer $k_i$, and each $t_{i,j}$ is an exponentially distributed random variable with rate $\lambda$.  Let $k= \max(k_1 , \ldots k_m)$, and $T=\max(t_1 ,\ldots t_m)$.  Then $E[T]=\Theta(k + \log m)$.
\end{lemma}
\begin{proof}
First we show that $E[T]=O(k+\log m)$.  Because of Ho-Lin, we know that $Pr[T>(1+\delta)] \leq m(\frac{1+\delta}{e^\delta})^k \leq m e^{-k\delta/2}$ for all $\delta \geq 3$.

Let $\delta_m = \frac{2 \ln m}{k}$.  Applying the above inequality we therefore get that:

$$ Pr[T > k(1 +\delta_m + x)] \leq e^{-kx/2}.$$

Therefore we know that:

$$ E[T] \leq k+2\ln m + \int_{x=0}^{\infty} e^{-kx/2} = O(k + \log m).$$


To show that $E[T] = \Omega(k + \log m)$, first note that $T \geq \max_{1\leq i\leq m} \{t_{i,1}\}$ and that $E[\max_{1\leq i\leq m}\{t_{i,1}\}] = \Omega(\log m)$, implying that $E[T] = \Omega(\log m)$.  Next, observe that $T \geq t_i$ for each $i$.  Since $E[t_i]$ is $k$ for at least one choice of $i$, we therefore get that $E[T] = \Omega(k)$.

\end{proof}


==> table.tex <==
\begin{table}[t] \label{tab:results}\caption{Summary of results.}
	\centering
	\begin{tabular}{|l||c c|c|}
		\hline
		~						& \multicolumn{2}{|c|}{Worst Case}				                         & Average Case				\\
& UB & LB & \\\hline\hline
&&&\\
		Addition(2D)			& \multicolumn{2}{|c|}{$\Theta(\sqrt{n})$} 	 & $O(\log{n})$ 				\\
&(Thm.\ref{thm:combinedAddition}) & (Thm.\ref{thm:addition} ) & (Thm.\ref{thm:combinedAddition}) \\ \hline
&&&\\
		Addition(3D)			& \multicolumn{2}{|c|}{$\Theta(\sqrt[3]{n})$} 	 & $O(\log{n})$ 				\\
& (Thm.\ref{thm:combined3d} ) & (Thm. \ref{thm:addition} ) & (Thm.\ref{thm:combined3d})\\ \hline
&&&\\
        Multiplication (3D) & $O(n^{\frac{5}{6}})$ & $\Omega(n^{\frac{1}{3}})$ & - \\
        & (Thm.~\ref{thm:56multiplication}) & (Thm.~\ref{thm:multiplication}) & \\ \hline
		Previous Best Addition(2D)		& $O(n)$ (See \cite{BRUN2007})	& \textbf{-} &	\textbf{-}			\\
		Previous Best Multiplication(2D)	& $O(n)$ (See \cite{BRUN2007}) 	& \textbf{-}	&	\textbf{-}		\\
		\hline
	\end{tabular}
\end{table}


==> tableNotBig.tex <==
\begin{table}[t] \label{tab:results}\caption{Summary of results.}
	\centering
	\begin{tabular}{|l|c c|c|}
		\hline
		~						& \multicolumn{2}{|c|}{Worst Case}				                         & Average Case				\\ \hline
		Addition(2D)			& \multicolumn{2}{|c|}{$\Theta(\sqrt{n})$} 	 & $O(\log{n})$ 				\\
&(Thm.\ref{thm:combinedAddition}) & (Thm.\ref{thm:addition} ) & (Thm.\ref{thm:combinedAddition}) \\ \hline
		Addition(3D)			& \multicolumn{2}{|c|}{$\Theta(\sqrt[3]{n})$} 	 & $O(\log{n})$ 				\\
& (Thm.\ref{thm:combined3d} ) & (Thm. \ref{thm:addition} ) & (Thm.\ref{thm:combined3d})\\ \hline
        Multiplication (3D) & $O(n^{\frac{5}{6}})$ & $\Omega(n^{\frac{1}{3}})$ & - \\
        & (Thm.~\ref{}) & (Thm.~\ref{thm:multiplication}) & \\ \hline
		Previous Best Addition(2D)		& $O(n)$ (See \cite{BRUN2007})	& \textbf{-} &	\textbf{-}			\\
		Previous Best Multiplication(2D)	& $O(n)$ (See \cite{BRUN2007}) 	& \textbf{-}	&	\textbf{-}		\\
		\hline
	\end{tabular}
\end{table}
